Optimizing Provenance Computations

Data provenance is essential for debugging query results, auditing data in cloud environments, and explaining outputs of Big Data analytics. A well-established technique is to represent provenance as annotations on data and to instrument queries to propagate these annotations to produce results annotated with provenance. However, even sophisticated optimizers are often incapable of producing efficient execution plans for instrumented queries, because of their inherent complexity and unusual structure. Thus, while instrumentation enables provenance support for databases without requiring any modification to the DBMS, the performance of this approach is far from optimal. In this work, we develop provenance specific optimizations to address this problem. Specifically, we introduce algebraic equivalences targeted at instrumented queries and discuss alternative, equivalent ways of instrumenting a query for provenance capture. Furthermore, we present an extensible heuristic and cost-based optimization (CBO) framework that governs the application of these optimizations and implement this framework in our GProM provenance system. Our CBO is agnostic to the plan space shape, uses a DBMS for cost estimation, and enables retrofitting of optimization choices into existing code by adding a few LOC. Our experiments confirm that these optimizations are highly effective, often improving performance by several orders of magnitude for diverse provenance tasks.

==> experiment_runtime_figs.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{figure*}[t]
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.4\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{
\footnotesize
%\subfloat[Sum]{
  \resizebox{0.55\linewidth}{!}{
  \begin{minipage}{1\linewidth}
  \begin{tabular}{|c|r|r|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
SAgg 1G & 4.79 & 20.21 & 4.38 & 2.69 & \textbf{0.81} \\ \hline 
SAgg 10G & 44.06 & 524.78 & 42.62& 27.47 & \textbf{7.65} \\ \hline 
    \hline
TPC-H 1G & $+$173,053.17 & \textbf{199.62} & 173,041.27 & 250.18 &  235.79 \\ \hline 
    TPC-H 10G & $+$175,371.02 & \textbf{2,033.71} & 175,530.53 & 2,247.39 & 2,196.01 \\ \hline
  \end{tabular}
\end{minipage}
}
%}
}
%%%%%%
{
\footnotesize
%\subfloat[Average]{
  \resizebox{0.55\linewidth}{!}{
  \begin{minipage}{1\linewidth}
  \begin{tabular}{|c|r|r|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
SAgg 1G & 1 & 3.927 & 0.946 & 0.600 & \textbf{0.261} \\ \hline 
SAgg 10G & 1 & 9.148 & 0.984 & 0.655 & \textbf{0.265} \\ \hline 
\hline
    TPC-H 1G & 1  & \textbf{0.187}  & 0.955 & 0.220 &  0.203\\ \hline 
TPC-H 10G & 1  & 0.198 & 0.975  & 0.180 & \textbf{0.174} \\ \hline
  \end{tabular}
\end{minipage}
}
%}
}
\caption{Total runtime (\textbf{Top}) and average runtime (\textbf{Bottom}) per query relative to NoHeu+Join for \textit{SimpleAgg} and \textit{TPC-H} workloads}
\label{tab:overview-sum-avg-sagg-tpch}
%\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.29\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_1GB_Combine.pdf}\\[-7mm]
  \caption{1GB \textit{SimpleAgg} Runtime}
  \label{fig:simpleAgg-comb-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.30\linewidth}
  \includegraphics[width=0.97\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_10GB_Combine.pdf}\\[-7mm] 
  \caption{10GB \textit{SimpleAgg} Runtime}
  \label{fig:simpleAgg-comb-10GB}
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%
\end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table*}
%\centering
%\begin{minipage}{0.49\linewidth}
%  \resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.1\linewidth}
%  \begin{tabular}{|c|r|r|r|r|r|} \hline 
%\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
%TPC-H 1G & $+$173,053.17 & \textbf{199.62} & 173,041.27 & 250.18 &  235.79 \\ \hline 
%TPC-H 10G & $+$175,371.02 & \textbf{2033.71} & 175,530.53 & 2,247.39 & 2,196.01 \\ \hline 
%SAgg 1G & 4.79 & 20.21 & 4.38 & 2.69 & \textbf{0.81} \\ \hline 
%SAgg 10G & 44.06 & 524.78 & 42.62& 27.47 & \textbf{7.65} \\ \hline 
%  \end{tabular}
%\end{minipage}
%}
%\caption{Total runtime for \textit{SimpleAgg} and \textit{TPC-H} workloads}
%\label{tab:overview-sum-sagg-tpch}
%\end{minipage}
%\begin{minipage}{0.49\linewidth}
%  \centering
%\resizebox{1\linewidth}{!}{
%  \begin{minipage}{1.1\linewidth}
%  \begin{tabular}{|c|r|r|r|r|r|} \hline 
%\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
%TPC-H 1G & 1  & \textbf{0.187}  & 0.955 & 0.220 &  0.203\\ \hline 
%TPC-H 10G & 1  & 0.198 & 0.975  & 0.180 & \textbf{0.174} \\ \hline 
%SAgg 1G & 1 & 3.927 & 0.946 & 0.600 & \textbf{0.261} \\ \hline 
%SAgg 10G & 1 & 9.148 & 0.984 & 0.655 & \textbf{0.265} \\ \hline 
%  \end{tabular}
%\end{minipage}
%}
%\caption{Average runtime per query relative to NoHeu+Join for \textit{SimpleAgg} and \textit{TPC-H}}
%\label{tab:overview-avg-simple-agg-tpch}
%\end{minipage}
%\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%\begin{figure*}[t]
%%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.49\linewidth}
%  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_1GB_Combine.pdf}\\[-7mm]
%  \caption{Runtime \textit{SimpleAgg} - 1GB}
%  \label{fig:simpleAgg-comb-1GB}  
%  \end{minipage}
%%%%%%%%%%%%%%%%%%%
%  \begin{minipage}[b]{0.49\linewidth}
%  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_10GB_Combine.pdf}\\[-7mm] 
%  \caption{Runtime \textit{SimpleAgg} - 10GB}
%  \label{fig:simpleAgg-comb-10GB}
%  \end{minipage}
%\end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/TPCH_1GB_Combine.pdf}\\[-7mm]
  \caption{Runtime \textit{TPC-H} - 1GB}
  \label{fig:tpch-comb-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/TPCH_10GB_Combine.pdf}\\[-7mm] 
  \caption{Runtime \textit{TPC-H} - 10GB}
  \label{fig:tpch-comb-10GB}
  \end{minipage}

  \begin{minipage}[b]{0.48\linewidth}
  \begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=1\linewidth,trim=0 70pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated.pdf}\\
  \vspace{-7mm}
  %\caption{Updates/Transaction and History Size}
  %\label{fig:Updates/Transaction-and-History-Size}
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=1\linewidth,trim=0 120pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated_overhead.pdf}\\
  \vspace{-7mm}
  %\caption{TransactionOverhead1}
  %\label{fig:Transaction Overhead: Updates/Transaction and History Size}
\end{minipage}
  \caption{Transaction provenance - runtime and overhead}
  \label{fig:Transaction-provenance-runtime}
\end{minipage}
  % \begin{minipage}[b]{0.48\linewidth}
% \includegraphics[width=1\linewidth,trim=0 20pt 0 30pt, clip]{figs/experiments_v1/numTupUpdated.pdf}\\
%   \vspace{-4mm}
%   %\caption{Number Updates/Transaction}
%   %\label{fig:Number-Updates/Transaction}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.25\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/export_15000r.pdf}\\[-7mm]
  \caption{Provenance Export}
  \label{fig:export}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.25\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/ProvenanceGame.pdf}\\[-7mm] 
  \caption{Datalog Provenance}
  \label{fig:provenance-game}
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%   

\end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \begin{figure*}[t]
%   \begin{minipage}[b]{0.48\linewidth}
%   \begin{minipage}[b]{0.48\linewidth}
% \includegraphics[width=1\linewidth,trim=0 70pt 0 30pt, clip]{figs/experiments_v1/uSizeNumTupUpdated.pdf}\\
%   \vspace{-7mm}
%   %\caption{Updates/Transaction and History Size}
%   %\label{fig:Updates/Transaction-and-History-Size}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.48\linewidth}
% \includegraphics[width=1\linewidth,trim=0 120pt 0 30pt, clip]{figs/experiments_v1/uSizeNumTupUpdated_overhead.pdf}\\
%   \vspace{-7mm}
%   %\caption{TransactionOverhead1}
%   %\label{fig:Transaction Overhead: Updates/Transaction and History Size}
% \end{minipage}
%   \caption{Transaction provenance - runtime and overhead}
%   \label{fig:Transaction-provenance-runtime}
% \end{minipage}
%   % \begin{minipage}[b]{0.48\linewidth}
% % \includegraphics[width=1\linewidth,trim=0 20pt 0 30pt, clip]{figs/experiments_v1/numTupUpdated.pdf}\\
% %   \vspace{-4mm}
% %   %\caption{Number Updates/Transaction}
% %   %\label{fig:Number-Updates/Transaction}
% %   \end{minipage}
% %   %%%%%%%%%%%%%%%%%%%% 
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.25\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/export_15000r.pdf}\\[-7mm]
%   \caption{Provenance Export}
%   \label{fig:export}  
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.25\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/ProvenanceGame.pdf}\\[-7mm] 
%   \caption{Datalog Provenance}
%   \label{fig:provenance-game}
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%%   
% \end{figure*}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "2016-prov-optimizer"
%%% End:


==> experiment_runtime_figs_2.tex <==
\begin{figure*}[p]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%       LEFT COLUMN
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{0.66\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=1\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_1GB_Combine.pdf}\\[-7mm]
  \caption{1GB \textit{SimpleAgg} Runtime}
  \label{fig:simpleAgg-comb-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=0.97\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_10GB_Combine.pdf}\\[-7mm] 
  \caption{10GB \textit{SimpleAgg} Runtime}
  \label{fig:simpleAgg-comb-10GB}
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=1\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/TPCH_1GB_Combine.pdf}\\[-7mm]
  \caption{Runtime \textit{TPC-H} - 1GB}
  \label{fig:tpch-comb-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=1\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/TPCH_10GB_Combine.pdf}\\[-7mm] 
  \caption{Runtime \textit{TPC-H} - 10GB}
  \label{fig:tpch-comb-10GB}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE 3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=1\linewidth,trim=0 60pt 0 100pt, clip]{figs/experiments_v2/export_15000r.pdf}\\[-7mm]
  \caption{Provenance Export}
  \label{fig:export}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.5\linewidth}
  \includegraphics[width=1\linewidth,trim=0 60pt 0 100pt, clip]{figs/experiments_v2/ProvenanceGame.pdf}\\[-7mm] 
  \caption{Datalog Provenance}
  \label{fig:provenance-game}
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE 4
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  
%%%%%%%%%%%%%%%%%%%%  
\begin{minipage}[b]{1\linewidth}  
%%%%%%%%%%%%%%%%%%%%  
\begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=1\linewidth,trim=0 -10pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated.pdf}\\
\vspace{-7mm}
%\caption{Updates/Transaction and History Size}
%\label{fig:Updates/Transaction-and-History-Size}
\end{minipage}
%%%%%%%%%%%%%%%%%%%% 
  \begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=1\linewidth,trim=0 0pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated_overhead.pdf}\\
  \vspace{-7mm}
  %\caption{TransactionOverhead1}
  %\label{fig:Transaction Overhead: Updates/Transaction and History Size}
\end{minipage}
  \caption{Transaction provenance - runtime and overhead}
  \label{fig:Transaction-provenance-runtime}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LINE 5
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%
  \begin{minipage}{1\linewidth}
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_overhead.pdf}\\[-7mm]
  %\caption{Simple Agg. Overhead}
  \label{fig:simple-agg-overhead}  
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 50pt 0 100pt, clip]{figs/experiments_v2/tpch_overhead.pdf}\\[-7mm] 
  %\caption{TPC-H Overhead}
  \label{fig:tpch-overhead}
  \end{minipage}
  \caption{\textit{SimpleAgg} (\textbf{Left}) and \textit{TPC-H} (\textbf{Right}) Overhead}
  \label{fig:simagg-tpch-overhead}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%       RIGHT COLUMN
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{0.33\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}{1\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \centering
\resizebox{1\linewidth}{!}{  
  \begin{minipage}{1.65\linewidth}
    \centering
  \begin{tabular}{|c|r|r|r|r|r|} \hline 
    \rowcolor[gray]{.9}   & \multicolumn{1}{|c|}{NoHeu}  & \multicolumn{1}{|c|}{NoHeu} & \multicolumn{1}{|c|}{Heu}  & \multicolumn{1}{|c|}{Heu}  & \multicolumn{1}{|c|}{Cost+Heu}\\
    \rowcolor[gray]{.9}   & \multicolumn{1}{|c|}{(Worst)} & \multicolumn{1}{|c|}{(Best)} & \multicolumn{1}{|c|}{(Worst)} & \multicolumn{1}{|c|}{(Best)} & \\
    \hline 
Min & 1.33 & 1.33 & \textbf{1.00} & \textbf{1.00} &  \textbf{1.00}\\ \hline 
Avg & 1,878.76 & 1,877.95 & 14.16 & 2.82 & \textbf{1.04} \\ \hline 
Max & $+$12,173.35& $+$12,173.35 & 68.63 & 7.80 & \textbf{1.18} \\ \hline 
  \end{tabular}
\end{minipage}
}\\[-1mm]
\caption{Min, max, and avg runtime relative  to the best method per workload aggregated over all workloads.}
\label{tab:overview-all}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{minipage}
%%%%%%%%%%%%%%%%%%%%
    \begin{minipage}{1\linewidth}
{
\footnotesize
%\subfloat[Sum]{
  \resizebox{0.6\linewidth}{!}{
  \begin{minipage}{1.1\linewidth}
  \begin{tabular}{|c|r|r|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
SAgg 1G & 4.79 & 20.21 & 4.38 & 2.69 & \textbf{0.81} \\ \hline 
SAgg 10G & 44.06 & 524.78 & 42.62& 27.47 & \textbf{7.65} \\ \hline 
    \hline
TPC-H 1G & $+$173,053.17 & \textbf{199.62} & 173,041.27 & 250.18 &  235.79 \\ \hline 
    TPC-H 10G & $+$175,371.02 & \textbf{2,033.71} & 175,530.53 & 2,247.39 & 2,196.01 \\ \hline
  \end{tabular}
\end{minipage}
}
%}
}\\[1mm]
%%%%%%%%%%%%%%%%%%%%
{
\footnotesize
%\subfloat[Average]{
  \resizebox{0.6\linewidth}{!}{
  \begin{minipage}{1.1\linewidth}
  \begin{tabular}{|c|r|r|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
SAgg 1G & 1 & 3.927 & 0.946 & 0.600 & \textbf{0.261} \\ \hline 
SAgg 10G & 1 & 9.148 & 0.984 & 0.655 & \textbf{0.265} \\ \hline 
\hline
    TPC-H 1G & 1  & \textbf{0.187}  & 0.955 & 0.220 &  0.203\\ \hline 
TPC-H 10G & 1  & 0.198 & 0.975  & 0.180 & \textbf{0.174} \\ \hline
  \end{tabular}
\end{minipage}
}
%}
}
\caption{Total runtime (\textbf{Top}) and average runtime (\textbf{Bottom}) per query relative to NoHeu+Join for \textit{SimpleAgg} and \textit{TPC-H} workloads}
\label{tab:overview-sum-avg-sagg-tpch}
%\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}

\begin{minipage}{1\linewidth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\resizebox{0.7\linewidth}{!}{  
  \begin{minipage}{1.45\linewidth}
    \centering
  \begin{tabular}{|c|r|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & FilterUpdated+NoHeu & HistJoin+Heu & FilterUpdated+Heu & Cost+Heu\\ \hline 
HSU/T & 55.11 & 69.50 &  \textbf{8.91} & \textbf{8.96} \\ \hline 
TAPU & 30.13 & 26.08 & \textbf{12.94} & \textbf{12.89} \\ \hline 
  \end{tabular}
\end{minipage}
}\\[-2mm]
\caption{Total workload runtime for transaction provenance}
\label{tab:overview-sum-transaction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{1\linewidth}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
  % $\,$\\[-3mm]
\resizebox{0.7\linewidth}{!}{
  \begin{minipage}{1.0\linewidth}
  \begin{tabular}{|c|r|r|r|} \hline 
\rowcolor[gray]{.9}  Queries & NoHeu & Heu & Cost+Heu \\ \hline 
Export 10M & 310.49 &  \textbf{0.25}&  \textbf{0.25} \\ \hline 
Export 100M & 3,136.94 & \textbf{0.27} &  \textbf{0.26}  \\ \hline 
Export 1G & +21,600 & \textbf{0.28} &  \textbf{0.28}   \\ \hline 
Export 10G & +21,600 & \textbf{3.03} & \textbf{3.01}  \\ \hline \hline
Datalog Provenance & 583.96 & 736.50 & \textbf{437.75} \\ \hline 
  \end{tabular}
\end{minipage}
}\\[-1mm]
\caption{Total runtime for export and Datalog workloads}
\label{tab:overview-sum-export-gp}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%% 
  \begin{minipage}[b]{1\linewidth}
  \includegraphics[width=1\linewidth,trim=0 0pt 0 20pt, clip]{figs/experiments_v2/simAggs_stack_m1.pdf}\\[-7mm]
  \caption{Optimization + runtime for Simple Agg. - 1GB}
  \label{fig:simAggs-all-stack}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{1\linewidth}
  \includegraphics[width=1\linewidth,trim=0 30pt 0 40pt, clip]{figs/experiments_v2/simpleAgg_sim_stack_m2.pdf}\\[-7mm] 
  \caption{Optimization + runtime for Simple Aggregation workload using Simulated Annealing - 1GB dataset}
  \label{fig:simple-agg-sim-annl}
  \end{minipage}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{minipage}
\end{figure*}

















% \begin{figure*}[t]
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% %\begin{figure*}[t]
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   % LINE 1
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_1GB_Combine.pdf}\\[-7mm]
%   \caption{1GB \textit{SimpleAgg} Runtime}
%   \label{fig:simpleAgg-comb-1GB}  
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=0.97\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_10GB_Combine.pdf}\\[-7mm] 
%   \caption{10GB \textit{SimpleAgg} Runtime}
%   \label{fig:simpleAgg-comb-10GB}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%
% %\end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \begin{minipage}{1\linewidth}
% \centering    
% {
% \footnotesize
% %\subfloat[Sum]{
%   \resizebox{0.45\linewidth}{!}{
%   \begin{minipage}{1\linewidth}
%   \begin{tabular}{|c|r|r|r|r|r|} \hline 
% \rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
% SAgg 1G & 4.79 & 20.21 & 4.38 & 2.69 & \textbf{0.81} \\ \hline 
% SAgg 10G & 44.06 & 524.78 & 42.62& 27.47 & \textbf{7.65} \\ \hline 
%     \hline
% TPC-H 1G & $+$173,053.17 & \textbf{199.62} & 173,041.27 & 250.18 &  235.79 \\ \hline 
%     TPC-H 10G & $+$175,371.02 & \textbf{2,033.71} & 175,530.53 & 2,247.39 & 2,196.01 \\ \hline
%   \end{tabular}
% \end{minipage}
% }
% %}
% }\\
% %%%%%%
% {
% \footnotesize
% %\subfloat[Average]{
%   \resizebox{0.45\linewidth}{!}{
%   \begin{minipage}{1\linewidth}
%   \begin{tabular}{|c|r|r|r|r|r|} \hline 
% \rowcolor[gray]{.9}  Queries & NoHeu+Join & Heu+Join & NoHeu+Window & Heu+Window & Cost+Heu\\ \hline 
% SAgg 1G & 1 & 3.927 & 0.946 & 0.600 & \textbf{0.261} \\ \hline 
% SAgg 10G & 1 & 9.148 & 0.984 & 0.655 & \textbf{0.265} \\ \hline 
% \hline
%     TPC-H 1G & 1  & \textbf{0.187}  & 0.955 & 0.220 &  0.203\\ \hline 
% TPC-H 10G & 1  & 0.198 & 0.975  & 0.180 & \textbf{0.174} \\ \hline
%   \end{tabular}
% \end{minipage}
% }
% %}
% }
% \caption{Total runtime (\textbf{Top}) and average runtime (\textbf{Bottom}) per query relative to NoHeu+Join for \textit{SimpleAgg} and \textit{TPC-H} workloads}
% \label{tab:overview-sum-avg-sagg-tpch}
% %\qquad\qquad\qquad\qquad\qquad\qquad\qquad\qquad
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{minipage}

% \begin{minipage}{1\linewidth}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%   \centering
% \resizebox{0.7\linewidth}{!}{  
%   \begin{minipage}{1.45\linewidth}
%     \centering
%   \begin{tabular}{|c|r|r|r|r|} \hline 
% \rowcolor[gray]{.9}  Queries & FilterUpdated+NoHeu & HistJoin+Heu & FilterUpdated+Heu & Cost+Heu\\ \hline 
% HSU/T & 55.11 & 69.50 &  \textbf{8.91} & \textbf{8.96} \\ \hline 
% TAPU & 30.13 & 26.08 & \textbf{12.94} & \textbf{12.89} \\ \hline 
%   \end{tabular}
% \end{minipage}
% }\\[-2mm]
% \caption{Total workload runtime for transaction provenance}
% \label{tab:overview-sum-transaction}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{minipage}
% \end{minipage}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


  
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LINE 2
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \begin{figure*}[t]
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/TPCH_1GB_Combine.pdf}\\[-7mm]
%   \caption{Runtime \textit{TPC-H} - 1GB}
%   \label{fig:tpch-comb-1GB}  
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/TPCH_10GB_Combine.pdf}\\[-7mm] 
%   \caption{Runtime \textit{TPC-H} - 10GB}
%   \label{fig:tpch-comb-10GB}
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/export_15000r.pdf}\\[-7mm]
%   \caption{Provenance Export}
%   \label{fig:export}  
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LINE 3
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.66\linewidth}
%   \begin{minipage}[b]{0.48\linewidth}
% \includegraphics[width=1\linewidth,trim=0 70pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated.pdf}\\
%   \vspace{-7mm}
%   %\caption{Updates/Transaction and History Size}
%   %\label{fig:Updates/Transaction-and-History-Size}
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.48\linewidth}
% \includegraphics[width=1\linewidth,trim=0 120pt 0 30pt, clip]{figs/experiments_v2/uSizeNumTupUpdated_overhead.pdf}\\
%   \vspace{-7mm}
%   %\caption{TransactionOverhead1}
%   %\label{fig:Transaction Overhead: Updates/Transaction and History Size}
% \end{minipage}
%   \caption{Transaction provenance - runtime and overhead}
%   \label{fig:Transaction-provenance-runtime}
% \end{minipage}
% %   %%%%%%%%%%%%%%%%%%%%   
%   \begin{minipage}[b]{0.33\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v2/ProvenanceGame.pdf}\\[-7mm] 
%   \caption{Datalog Provenance}
%   \label{fig:provenance-game}
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%%   

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % LINE 4
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%
%   \begin{minipage}{0.66\linewidth}
%   \begin{minipage}[b]{0.49\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 70pt 0 100pt, clip]{figs/experiments_v2/simpleAgg_overhead.pdf}\\[-7mm]
%   %\caption{Simple Agg. Overhead}
%   \label{fig:simple-agg-overhead}  
%   \end{minipage}
%   %%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.49\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 70pt 0 100pt, clip]{figs/experiments_v2/tpch_overhead.pdf}\\[-7mm] 
%   %\caption{TPC-H Overhead}
%   \label{fig:tpch-overhead}
%   \end{minipage}
%   \caption{\textit{SimpleAgg}(\textbf{Left}) and \textit{TPC-H}(\textbf{Right}) Overhead}
%   \label{fig:simagg-tpch-overhead}
% \end{minipage}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{minipage}{0.33\linewidth}
% %%%%%%%%%%%%%%%%%%%% 
%   \begin{minipage}[b]{1\linewidth}
%   \includegraphics[width=1\linewidth,trim= 0 10pt 0 0pt, clip]{figs/experiments_v2/simAggs_stack.pdf}\\[-7mm]
%   \caption{Optimization + runtime for Simple Agg. - 1GB}
%   \label{fig:simAggs-all-stack}  
%   \end{minipage}
% %%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{1\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 80pt 0 80pt, clip]{figs/experiments_v2/simpleAgg_sim_stack.pdf}\\[-7mm] 
%   \caption{Optimization + runtime for Simple Aggregation workload using Simulated Annealing - 1GB dataset}
%   \label{fig:simple-agg-sim-annl}
%   \end{minipage}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \end{minipage}

% \end{figure*}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "2016-prov-optimizer"
%%% End:


==> experiments.tex <==

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]

%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.33\linewidth}
  \includegraphics[width=1\linewidth,trim=0 70pt 0 70pt, clip]{figs/experiments_v1/simpleAgg_1GB.pdf}\\[-5mm]
  \caption{Simple Agg. - 1GB}
  \label{fig:simple-agg-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.33\linewidth}
  \includegraphics[width=1\linewidth,trim=0 70pt 0 70pt, clip]{figs/experiments_v1/simpleAgg_10GB.pdf}\\[-5mm]
  \caption{Simple Agg. - 10GB}
  \label{fig:simple-agg-10GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.33\linewidth}
  \includegraphics[width=1\linewidth,trim=0 70pt 0 120pt, clip]{figs/experiments_v1/simpleAgg_overhead.pdf}
  \caption{Simple Agg. - Opt. Overhead}
  \label{fig:SimpleAgg Overhead}  
  \end{minipage}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v1/tpch_1GB.pdf}\\[-7mm]
  \caption{TPC-H Queries - 1GB}
  \label{fig:tpch-1GB}  
  \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 80pt 0 100pt, clip]{figs/experiments_v1/tpch_10GB.pdf}\\[-7mm] 
  \caption{TPC-H Queries - 10GB}
  \label{fig:tpch-10GB}
  \end{minipage}
% \end{figure*}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[t]
%%%%%%%%%%%%%%%%%%%%
  % \begin{minipage}[b]{0.49\linewidth}
  % \includegraphics[width=1\linewidth,trim=0 70pt 0 70pt, clip]{figs/experiments_v1/TPCH_average1.pdf}
  % \caption{TPC-H factor 1}
  % \label{fig:TPCH-factor1}  
  % \end{minipage}
%%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.49\linewidth}
  \includegraphics[width=1\linewidth,trim=0 90pt 0 120pt, clip]{figs/experiments_v1/tpch_overhead.pdf}
  \caption{TPC-H - Optimization Overhead}
  \label{fig:TPCH Overhead}  
  \end{minipage} 
 \begin{minipage}[b]{0.49\linewidth}
    \centering
  \includegraphics[width=0.7\linewidth,trim=0 70pt 0 70pt, clip]{figs/experiments_v1/TPCH_average2.pdf}
  \caption{TPC-H - Average Performance Relative to Best}
  \label{fig:TPCH-factor2}  
  \end{minipage}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}\label{sec:experiments}

Our experimental evaluation focuses on  evaluating 1) the effectiveness of cost-based optimization in choosing the best alternative, 2) the effectiveness of provenance specific transformations, and 3) the overhead incurred by our heuristic and cost-based optimizations.
% 3) estimate the runtime overhead paid to provenance specific transformation rules and cost-based optimization.
All experiments were executed on a  machine with 2 AMD Opteron 4238 CPUs, 128GB RAM, and a hardware RAID with  4 $\times$ 1TB 72.K HDs in RAID 5.

% the configuration shown in Table~\ref{tab:exp-config}.

% %%%%%%%%%%%%%%%%%%%%
% \begin{table}[t]
% \centering
%   \begin{tabular}{|c|c|} \hline 
%   \rowcolor[gray]{.9}  Name & type \\ \hline 
%   CPUs & 2 $\times$ AMD Opteron 4238 (12 cores)   \\ \hline
%   RAM & 128 GB   \\ \hline
%   Hardware & 4 $\times$ 1TB 7.2K HDs   \\ \hline
%   \end{tabular}
% \caption{Experiment configuration}
% \label{tab:exp-config}
% \end{table}
% %%%%%%%%%%%%%%%%%%%%



%\subsection{Datasets}

% We use two types of datasets in our experiments that are described below.

% \noindent\textbf{TPC-H benchmark: }
%  We use the TPC-H benchmark to test our cost-based optimization. 
% \BG{Cite}
% The TPC-H benchmark is a decision support benchmark. It is consists of suite of bussiness oriented ad-hoc queries and concurrent data modifications.
%  The queries and the data populating the database have been chosen to have broad industry-wide relevance while maintaining a sufficient degree of ease of implement. This benchmark has following three features: large volumes of data and 
%  queries with a high degree of complexity~\cite{tpch}. We generated TPC-H benchmark conformant datasets of size 10MB, 100MB, 1GB, and 10GB respectively. 

%\noindent\textbf{Synthetic Datasets: }
% In addition to the TCP-H experiments, we also tested our optimization on synthetic data. The goal is to discover potential optimizations.
% We use a relation with five numeric
%columns. Values for these attributes are chosen from a uniform distribution. 
%We created variants $R10K$, $R100K$, and $R1000K$ with 10K, 100K, 1M tuples and no significant history ($H0$). Additionally, we generated three variants  of $R1000K$ with different history sizes $H10$, $H100$, and $H1000$ (100K, 1M, and 10M tuples history).
%At first,   we only consider transactions that
%consist solely of update statements. 
%We vary the following parameters: $U$ is the number of updates per
%transaction, e.g., $U10$ is a transaction with 10 updates. $T$ is the number
%tuples affected by each update. Unless stated otherwise, we use $T1$. The tuple
%to be updated is selected using the primary key.
%All transactions were executed under 
%isolation level 
%\texttt{SERIALIZABLE} (\textit{SI}). 



%\subsection{Workloads}

%\begin{itemize}
% \item \textbf{Simple aggregation queries: }
% In our cost-based optimization experiments, the performance of nested aggregation operations is tested. An aggregation test query consists of \textit{agg} aggregation operations. Each
%aggregation operates on the result of its child aggregation. The leaf operation accesses the TCP-H table part. Every aggregation groups the input on a range of primary key attribute values.
%The ranges are chosen so that each operation performs approximately the same number of aggregation function computations. This is achieved by grouping on the primary key attribute divided by
%$numGrp =  \sqrt[agg]{|part|} $. 
% \item \textbf{Transactional workload: }
%\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Experimental results}


% \subsection{Placeholder}
% \begin{itemize}
% \item
% \item
% \item
% \end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Cost-based Optimization}
% \subsection{Compare methods}

To evaluate how effectiveness of  our cost-based optimizer in choosing the lowest cost alternative and how our provenance specific transformation rules improve the performance, we compared the performance of queries generated by the cost-based optimizer against queries generated by taking a predetermined choice during provenance rewrite.
% For provenance specific transformation rules, we we compared the performance of queries which activated these rules with deactivated these rules.
We focus on following choices introduced in Sec.~\ref{sec:transf-appl-during}: 1) using the (\textbf{\textit{Window}}) or  (\textbf{\textit{Join}}) method for  rewriting an aggregation operator for provenance computation and 
2) Filtering tuples updated by a transaction using selection conditions (\textbf{\textit{FilterUpdated}}) or a temporal join (\textbf{\textit{HistJoin}}) compute of provenance of transactions. \textbf{\textit{Cost}} is our cost-based optimization which choose the cheapest method between (\textbf{\textit{Window}}) and (\textbf{\textit{Join}})
or between (\textbf{\textit{FilterUpdated}}) and (\textbf{\textit{HistJoin}}). For each one, we activate provenance specific transformation rules (suffix \textbf{\textit{Opt}} is added to the name) and deactivate provenance specific transformation rules (\textbf{\textit{NoOpt}}).  
%We also compared \textit{joinNoOpt} and \textit{windowNoOpt} which are deactivating the heuristic optimizaion respectively.  
% Here we use both simple aggregation queries and TPC-H queries - both executed over TPC-H datasets. 

%For this experiment we use a workload of provenance computations
%for transactions.

\subsection{Datasets and Workload}

%\subsubsection{Dataset}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{TPC-H datasets}
%For this experiment we use TPC-H datasets. 
The TPC-H benchmark is a standard decision support benchmark. % It is consists of suite of bussiness oriented ad-hoc queries and concurrent data modifications.
% The queries and the data populating the database have been chosen to have broad industry-wide relevance while maintaining a sufficient degree of ease of implement.
% This benchmark has following features: large volumes of data and 
% queries with a high degree of complexity.
We generated TPC-H benchmark datasets of size 10MB, 100MB, 1GB, and 10GB. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{Synthetic dataset}
For transaction provenance experiments we use a relation with five uniformly distributed numeric attributes. 
We created variants $R10K$, $R100K$, and $R1000K$ with 10K, 100K, 1M tuples. For
$R1000K$ we created different sizes of transactional history (this affects
performance, because the database has too store this history to enable time
travel that we need to compute provenance for transactions). Parameter $HX$
indicates $X\%$ of history, e.g., $H10$ represent $10\%$ history
which amounts to 100K tuples for relation $R1000K$. 
 
%\subsubsection{Workloads}
%We use three workloads in this experiment. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{Simple aggregation queries}
This workloads computes the provenance of queries consisting solely of aggregation operations. An aggregation  query consisting of $i$ aggregation operations where each
aggregation operates on the result of the previous aggregation. The leaf operation accesses the TPC-H part table. Every aggregation groups the input on a range of primary key attribute values such that the last step returns the same number of results independent of $i$. 
% The ranges are chosen so that each operation performs approximately the same number of aggregation function computations. This is achieved by grouping on the primary key attribute divided by
% $numGrp =  \sqrt[agg]{|part|} $. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{TPC-H queries}
The TPC-H benchmark consists of 22 queries. We have selected 11 representative queries to evaluate the optimizer over provenance computation for complex queries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{Transactions}
We consider provenance computations for transactions that consist solely of
update statements.  We vary the following parameters: $U$ is the number of
updates per transaction, e.g., $U10$ is a transaction with 10 updates. $T$ is
the number tuples affected by each update. Unless stated otherwise, we use
$T1$. The tuples to be updated are selected randomly using the primary key of
the relation.  All transactions were executed under isolation
level~\texttt{SERIALIZABLE}. 

% Note that these transaction do not exhibit the
% exponential expression growth problem we mentioned in the introduction. Our
% optimizations can deal with such queries. However, we wanted to compare to the
% performance of unoptimized provenance computations which would not be possible
% for such queries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}[t]
%%%%%%%%%%%%%%%%%%%% 
  \begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1\linewidth,trim=0 10pt 0 30pt, clip]{figs/experiments_v1/uSizeNumTupUpdated.pdf}\\
  \vspace{-4mm}
  %\caption{Updates/Transaction and History Size}
  %\label{fig:Updates/Transaction-and-History-Size}
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1\linewidth,trim=0 20pt 0 30pt, clip]{figs/experiments_v1/numTupUpdated.pdf}\\
  \vspace{-4mm}
  %\caption{Number Updates/Transaction}
  %\label{fig:Number-Updates/Transaction}
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%% 
  \begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1\linewidth,trim=0 20pt 0 30pt, clip]{figs/experiments_v1/uSizeNumTupUpdated_overhead.pdf}\\
  \vspace{-4mm}
  %\caption{TransactionOverhead1}
  %\label{fig:Transaction Overhead: Updates/Transaction and History Size}
  \end{minipage}
  %%%%%%%%%%%%%%%%%%%%
  \begin{minipage}[b]{0.24\linewidth}
\includegraphics[width=1\linewidth,trim=0 20pt 0 30pt, clip]{figs/experiments_v1/numTupUpdated_overhead.pdf}\\
  \vspace{-4mm}
  %\caption{TransactionOverhead2}
  %\label{fig:Transaction Overhead Number Updates/Transaction}
  \end{minipage}

  \caption{Transaction provenance}
  \label{fig:Transaction provenance}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[t]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\parttitle{Simple Aggregation Queries. } 
We measure the runtime of computing the provenance of the simple aggregation queries over the 1GB and 10GB TPC-H datasets. 
%datasets of size 10MB up to 10GB. % Because the number of pages is limited, we only show the results in datasets size 1GB and 10GB 
%Fig.~\ref{fig:simple-agg-10MB} to \ref{fig:simple-agg-10GB} shows the results of computing the provenance of the simple aggregation queries use datasets of size 10MB up to 10GB.
We vary the number of aggregation in the query and compare runtime of the \textit{Cost+Opt}, \textit{Window+Opt}, \textit{Join+Opt}, \textit{Window+NoOpt} and \textit{Join+NoOpt} methods mentioned above.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Simple Aggregation Queries}
%\label{sec:simple-aggr-quer}
%In this experiment we computed the provenance of the simple aggregation queries use datasets of size 10MB up to 10GB. 
%We vary the number of aggregation in the query and compare runtime of the \textit{cost}, \textit{window}, \textit{join}, \textit{windowNoOpt} and \textit{joinNoOpt} methods mentioned above.
%The results of this experiment are shown in Fig.~\ref{fig:simple-agg-10MB} to \ref{fig:simple-agg-10GB} (the data set sizes are 10MB, 100MB, 1GB, and 10GB).  
The median runtimes over 100 runs are shown in Fig.~\ref{fig:simple-agg-1GB} and~\ref{fig:simple-agg-10GB}. Note that the y-axis is log-scale.
% In these figures, the vertical axis shows the running time in seconds (logarithmic scale) whereas the horizontal axis indicates the number of aggregations ranging from 1 to 10.
The \textit{Window} method outperforms the \textit{Join} method by several orders of magnitude for larger number of aggregations. This is not surprising, because the \textit{Join} method increases the query size by a factor that is quadratic in the number of aggregation operators found on any path between the root of an algebra graph and a leaf node. Activating heuristic optimizations improves performance in most cases, but for this workload the dominating factor is the method used for rewriting aggregations. The only exceptions are \textit{Join} rewrites for the 1GB dataset. Here, performance decreases if the heuristic optimizations are activated. We inspected the plans used by the backend DBMS. A suboptimal join order was chosen for \textit{Join+Opt} based on inaccurate estimations of intermediate result sizes. For \textit{Join} the database did not remove unnecessary intermediate operators that blocked join reordering and, thus, executed the joins in the order provided in the input query which turned out to be more efficient in this case.
%
% We can see in Fig.~\ref{fig:simple-agg-1GB} \textit{Window+Opt} always get better performance than \textit{Window} which shows our provenance specific transformation rules always improve the performance.
% But in Fig.~\ref{fig:simple-agg-10GB}, the \textit{Join} get better performance than \textit{Join+Opt}. This is because the database 
% generated the different plans and materialized the subquery of \textit{Join}. For cost-based method, we can see that window method consistently outperforms the join based method whatever with \textit{Opt} or with \textit{NoOpt} except for only with 1 or 2 aggregations.
% The window based method is several orders of magnitude faster than the join method for larger database sizes and higher number of aggregations.
%
Consistently, the cost-based method was either able to select \textit{Window} as the superior method (we confirmed this by inspecting the generated plan) or to outperform both \textit{Window} and \textit{Join}.
% In some cases we can see the cost-based optimizer was able to generate a query that is cheaper than both the join and window method. % for example in 
%Fig.~\ref{fig:simple-agg-10GB}.
This is, because the cost-based optimizer was able to determine that the best plan for these queries is created by rewriting some of the aggregations in a query using  \textit{Window} and others with \textit{Join}.
% This is because there are several levels of aggregations in the query, the cost-based method can always choose the best method in different levels.
% In any figures, our \textit{Cost+Opt} always outperform than any other method.
Note that in Fig.~\ref{fig:simple-agg-10GB}, that the missing results (\textit{Join} for 6 levels of aggregation) are due to a suboptimal plan. These queries did not finish execution within 1 hour.

In Fig.~\ref{fig:SimpleAgg Overhead}, we show the overhead incurred activating/deactivating certain optimization methods. 
%  activating provenance specific transformation rules with deactivating provenance specific transformation rules, we also compared them with cost-based
% method which with \textit{Opt} and with \textit{NoOpt}.
Heuristic optimization (\textit{Opt}) results in an overhead of $\sim50$ ms  compared to the time of compiling the provenance request without any optimization (\textit{NoOpt}) and this overhead is only slightly affected by the number of aggregations in the query. When increasing the number of aggregations,
the running time of \textit{Cost} increases more significantly because we have 2 choices for each aggregation, i.e., the plan space size is $2^{i}$ for $i$ aggregations. % which because more layers of aggregations means we can generate more plans. 
We measure where time is spend during cost-based optimization and determined that the majority of time is spend in costing SQL queries using the backend DBMS. Note that even though we did not apply any techniques to  reduce the search space (randomized search or our techniques that adapts optimization time based on expected runtime), the sum of optimization time and runtime for \textit{Cost} is still less than this sum for the \textit{Join} method in all cases.
% ADD ARGUMENT ABOUT WHAT TO DO HERE
% we do not report results for the \textit{Join} and \textit{Join+NoOpt} methods join based methods of 6 levels of aggregation , because they did not finish within 1 hour. The reason % reasonable time (we interrupted queries running 
% longer than 1 hour).


 % able to recognize the best method showing the same performance as the window method. We manually confirmed that in all these cases the query generated by the cost-based optimizer was the same as the one produced by the window method. 
%  From the result, cost-based does what we supposed to do, the window based one
% is much better than join based one, the cost-based optimizer makes the correct choice.




 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure*}[t]

% %%%%%%%%%%%%%%%%%%%%
%   \begin{minipage}[b]{0.49\linewidth}
%   \includegraphics[width=1\linewidth,trim=0 90pt 0 120pt, clip]{figs/experiments_v1/tpch_overhead.pdf}
%   \caption{TPC-H - Overhead}
%   \label{fig:TPCH Overhead}  
%   \end{minipage}

% \end{figure*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{TPC-H Queries}
%\label{sec:simple-aggr-quer}
\parttitle{TPC-H Queries} 
We use provenance computations for TPC-H queries to determine whether the results for the simple aggregation queries translate to more complex queries. % and to confirm that there are workloads on which choosing the join method is beneficial.
The results for 1GB and 10GB are shown in Fig.~\ref{fig:tpch-1GB} and~\ref{fig:tpch-10GB}. % here we also only shows the results in database size 1GB and 10GB. 
% In these two figures, the vertical axis still shows the running time whereas the horizontal axis indicates the query.
% Here we use the queries Q1, Q5, Q10 and Q13, because some problem of the Q5 and Q10, we only shows the result of Q1 and Q13 which already give the nice results.
Depending on the dataset and query, there are cases where the \textit{Join} method is superior and others where the \textit{Window} method is superior. Also the runtime difference between these methods are less extreme presenting a challenge for our cost-based optimizer. 
Nonetheless, the cost-based method has the same cost as the cheapest method in almost all cases. 
We also get the results of \textit{NoOpt} for each method for the 1GB dataset. However, only two queries finished in the allocated time slot of 1 hour (Q1 within 226.28 seconds and Q13 within 216.89 seconds). Thus, the TPC-H workload demonstrates the need for heuristic optimizations and the robustness of our cost-based optimizer.
% and the \textit{Opt} outperforms than \textit{NoOpt} expecially in large size dataset.

% In Fig.~\ref{fig:TPCH Overhead} and Fig.~\ref{fig:SimpleAgg Overhead}, we use TPCH queries and simple aggregations to test the overhead of our optimizer.

In Fig.~\ref{fig:TPCH Overhead}, we show the overhead of each  optimization method on provenance rewriting. Activating heuristic optimization results in roughly $50ms$ overhead in most cases with a maximum overhead of $\sim0.5sec$. Cost-based optimization takes up to 3 seconds in the worst case. This is more than offset by the gain query performance (recall that without heuristic optimization only 2 queries finish within 1 hour over the 1GB dataset). 
%  window method, join method and cost-based method all with \textit{Opt} and with \textit{NoOpt}. We can see \textit{Opt} cost a little bit than \textit{NoOpt} in 
% every methods \textit{Window}, \textit{Join} and \textit{Cost}. The \textit{Cost} cost more than other methods because its time spend on the estimating the running time. The cost-based method generated many plans and each plan needs database to give an estimated cost. 


Provenance computations for different TPC-H queries show quite diverse runtimes. To gain insights into the performance gained though cost-based optimization without having expensive queries dominating the results, we computed for each query the relative overhead of a method compared to the cheapest method for this query. For example, a factor $1.1$ would mean that the method was 10\% slower than the best method (for this particular query) and a factor $1$ would indicate that this method is the best for this query.
Fig.~\ref{fig:TPCH-factor2} shows the average relative overhead. \textit{Join} is on average $\sim 50\%$ worth than the best method for 1GB and this factor increases to almost 2 for 10GB. For window we see an increase from $\sim 20\%$ to about $30\%$. The average performance benefits of \textit{Cost} increase with the dataset size (the overhead drops from $\sim 13\%$ to $\sim 10\%$).
% This is likely due to the fact that choosing

%  each TPCH queries as the standard and get the relative value of each method compared to the standard for every TPCH queries. Then we sum the relative value of each method and divide by the number of the TPCH queries.
% We can see the Cost-based method always get better performance compared with the most costly one and sometimes get better performance than both, for example in 1GB and 10GB size.


% Fig.~\ref{fig:TPCH-factor1}, we sum the minimum runtime of each TPCH queries and use this value as a standard. Then we get the sum runtime of window, join and cost respectively and divide by the standard.
% We can see the Cost-based method always get better performance compared with the most costly one and sometimes get better performance than both, for example in 10GB size.

% Fig.~\ref{fig:TPCH-factor2}, we use the minimum runtime of each TPCH queries as the standard and get the relative value of each method compared to the standard for every TPCH queries. Then we sum the relative value of each method and divide by the number of the TPCH queries.
% We can see the Cost-based method always get better performance compared with the most costly one and sometimes get better performance than both, for example in 1GB and 10GB size.


%However, there are two exceptions.
%For query Q13 in Fig.~\ref{fig:tpch-1GB}, the cost-based methods shows a runtime that lies between the join method and window method. This is because the database cost model is not perfect, which mislead our optimizer to think that a combination of both methods (each applied for one of the two aggregations in the query) would have the lowest cost. The second exception is query Q13 over the 10GB instance (Fig.~\ref{fig:tpch-10GB}). Here the cost-based optimizer was able to generate a query that is cheaper than both the join and window method. Here the optimizer has chosen to apply the join method for one aggregation in query Q13 and the window for the other. In summary, this experiment demonstrates that our optimizer outperform purely heuristic choices and is able to determine which choice is better even if the performance differences are not as significant as in the previous experiment.
%For query Q5 in Fig.~\ref{fig:tpch-1GB}, here the cost-based optimizer was able to generate a query that is cheaper than both the join and window method. Here the optimizer has chosen to apply the join method for one aggregation in query Q5 and the window for the other. In summary, this experiment demonstrates that our optimizer outperform purely heuristic choices and is able to determine which choice is better even if the performance differences are not as significant as in the previous experiment.





 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Heuristic Optimization}

%Here we use three configuration to test the effectiveness of our heuristic
%rules: applying no heuristic optimizations at all, active heuristic
%optimizations except for projection merging, and active all heuristic
%optimizations. For this experiment we use a workload of provenance computations
%for transactions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Datasets}
%Here we use synthetic datasets. We use a relation with five numeric
%attributes. Values for these attributes are chosen from a uniform distribution.
%We created variants $R10K$, $R100K$, and $R1000K$ with 10K, 100K, 1M tuples. For
%$R1000K$ we created different sizes of transactional history (this affects
%performance, because the database has too store this history to enable time
%travel that we need to compute provenance for transactions). Parameter $H0$
%indicates no significant history whereas $H1000$ represent $1000\%$ history
%which amounts to 10M tuples in case of relation $R1000K$. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Workloads}
%We consider provenance computations for transactions that consist solely of
%update statements.  We vary the following parameters: $U$ is the number of
%updates per transaction, e.g., $U10$ is a transaction with 10 updates. $T$ is
%the number tuples affected by each update. Unless stated otherwise, we use
%$T1$. The tuples to be updated are selected randomly using the primary key of
%the relation.  All transactions were executed under isolation
%level~\texttt{SERIALIZABLE}. Note that these transaction do not exhibit the
%exponential expression growth problem we mentioned in the introduction. Our
%optimizations can deal with such queries. However, we wanted to compare to the
%performance of unoptimized provenance computations which would not be possible
%for such queries.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsubsection{Results}
\parttitle{Transactions}
We next compute the provenance of transactions using the techniques introduced in~\cite{AG16a}. We vary the number of updates per
transaction ($U1$, $U10$, $U100$, and $U1000$) and the size of the database
($H10$, $H100$, and $H1000$).  The results are shown in the left two graphs in Fig.~\ref{fig:Transaction provenance}. % shows the results of transaction provenance. 
%We use \textit{NoOpt} which denotes non
%heursitic optimization, \textit{OptNoMerg} which denotes applying all heuristic
%optimization rules without the merge rule and \textit{Opt} which denotes
%applying all heuristic optimizaion rules.

%Fig.~\ref{fig:No Significant History} shows the runtime of these provenance
%computations over relations with no significant history ($H0$).  We scale
%linearly in $R$ and $U$. By reducing the amount of data to be processed by the
%reenactment query, without applying the merge rule, \textit{OptNoMerge} can
%always get better performance than \textit{NoOpt}.  By applying projection
%merging, the performance of \textit{Opt} is largely improved compared to
%\textit{OptNoMerge}.

The leftmost graph shows results for varying the
number of updates ($U1$, $U10$, $U100$ and $U1000$) using \textit{R1000K-H10}, \textit{R1000K-H100} and \textit{R1000K-H1000}.
We compared the performance of \textit{FilterUpdated+NoOpt}, \textit{FilterUpdated+Opt}, \textit{MergingHistJoin+Opt}, and \textit{Cost+Opt}. 
Our cost-based optimizer did correctly choose \textit{FilterUpdated+Opt} as the better alternative for this workload. 
% this optimization is
% more effective for larger transactions, because the reenactment queries for such
% transactions are increasingly complex.
\textit{FilterUpdated+Opt} exhibits better performance than
\textit{FilterUpdated+NoOpt} and this performance gap  increases with the number of the updates per transaction. 
%the performance was improved largely. 
% textit{Cost+Opt} always choose similar with the \textit{FilterUpdated+Opt}.
%Except for the last one $U1000$, \textit{Opt} get better performance
%than \textit{OptNoMerge}. The \textit{NoOpt} configuration did not finish without a 1 hour threshold.

The second plot from the left in   Fig.~\ref{fig:Transaction provenance} show results for $U50$
where each update modifies 10, 100, 1000 or 10000 tuples of relation
\textit{R1000K-H1000}. As evident from this graph, the runtime is not significantly affected when increasing the number
of affected tuples per update. 
%Heuristic optimization always shows better performance than
%heuristic optimization without merging projections.  And active heuristic optimizaion without
%merge can always get better than applying no optimization. Merging projections is quite effective for large number of updates per transactions.
The \textit{FilterUpdated+Opt} performs better  than
\textit{FilterUpdated+NoOpt} and \textit{Cost+Opt} always picked the best choice  (\textit{FilterUpdated+Opt}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\parttitle{Overhead}

The right two graphs in Fig.~\ref{fig:Transaction provenance} show the overhead of the compared methods for the transaction provenance computations from the left two plots of this figure.  % which corresponds to the left two transaction provenance graphs respectively. 
%Fig.~\ref{fig:Transaction Overhead Number Updates/Transaction} and~\ref{fig:Transaction Overhead: Updates/Transaction and History Size} shows the overhead of transactions which shows in Fig.~\ref{fig:Number-Updates/Transaction} and~\ref{fig:Updates/Transaction-and-History-Size} respectively. 
The overhead increases for larger transactions (larger $U$ values), but even though optimization time becomes a significant factor, optimization time is still offset by savings in query time.
% We can see \textit{Opt} still cost a little bit than \textit{NoOpt} and \textit{Cost} cost than other methods. 

\subsection{Summary}
Our experiments confirm the effectiveness of our provenance specific transformation rules and cost-based optimization method - often improving performance by several orders of magnitude. Our cost-based optimizer was able to pick the right alternatives in almost all cases.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "2016-prov-optimizer"
%%% End:


==> implementation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Implementation}\label{sec:overview}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the following I will separately present our heuristic and cost-based optimization techniques. In this section I give a brief overview of how these techniques interact and how they have been implemented in the GProM system. We apply heuristic rewrites to the AGM graph after it has been rewritten by the provenance rewriter module (compare Fig.~\ref{fig:GProm-arch}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{The GProM System}
%\label{sec:gprom-system}

GProM (\textbf{G}eneric \textbf{Pro}venance \textbf{M}iddleware) is a middleware system that enables computation of provenance for queries, updates, and transactions over several database backends (e.g., Oracle).
GProM is the first system capable of computing the provenance of 
concurrent database transactions. 
 It uses annotation propagation and query rewrite techniques for
computing, querying, storing, and translating the provenance of SQL queries, updates, transactions, and across transactions. % Also, it is database independent and 
% support multiple provenance computation.
% It uses the query rewrites technique 
% which from rewriting the algebra query tree and then translate it into 
% SQL code. 
Internally all queries are represented as relational algebra graphs in GProM. Fig.~\ref{fig:GProm-arch} shows the architecture of the system. User queries (including requests for provenance) are parsed and transformed into relational algebra graphs. We refer to this representation as \textit{AGM} (algebra graph model). The provenance rewrite techniques that take the input request and rewrite it to propagate provenance all operate on the AGM representation of a query. 
The  heuristic 
and cost-based optimizations presented in this paper also operate on AGM graphs.
After a query is optimized by our optimizer, the AGM graph is translated into executable SQL code in the dialect of the backend database system. 
The  ultimate goal of my work is to develop an optimizer module that can be used to improve the performance of different types of provenance computations. GProM is an ideal platform for this type of research, because it already support several different provenance types  (e.g., provenance for queries using the semiring model~\cite{karvounarakis2012semiring}, the first implementation of provenance for transactions, and game provenance~\cite{KL13}) and backend languages (currently Oracle's SQL dialect and datalog).
Since database systems already employ quite evolved optimization techniques, it is essential that the proposed optimizations do not hinder the database optimizer in exploring its plan search space. 
In the following, I will provide examples to help the reader understand some of the provenance types supported by  GProM. 

%  generated SQL 
% code can be successfully optimized by the underlying DBMS. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

If cost-based optimization is deactivated then the result of the heuristic optimizations is passed to the SQL code generators executed on the backend database. If cost-based optimization is activated then the cost-based optimizer takes the AGM graph generated by the parser and repeatedly runs this graph though the provenance rewriter, heuristic optimization, and SQL code generation modules to generate multiple SQL queries (``plans''). This is achieved by forcing these modules to make different choices in each iteration. Each generated query is costed using the backend database and eventually the query with the lowest estimated cost is executed. Since it is our goal to minimize the query runtime experienced by the user of our system (which includes both the time we spend on optimization and the time we spend on executing the query) we may decide to stop optimization once we have found a plan that is ``cheap enough''.



% Our work is based on the GProM system which is the first system to support provenance computation for concurrent transactions by using SQL rewrite techniques. However, it faces the same problem with other rewrite based provenance computation systems that the new generated queries are hard to be optimized by normal database optimizers. Thus we introduce an optimizer which based on heuristic and cost-based methods to deal with these complex queries. For some queries we make sure it can get a better performance by using some heuristic rules, but for some other heuristic rules, we are not sure if it can get a better performance, so we add the cost-based optimizer and let the database itself to decide if this rule can get a better performance. At last, we use experiment to evaluate our work and the result shows that our work can successfully optimize the complex queries.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "2016-prov-optimizer"
%%% End:

